Geometry-Entangled Visual Semantic Transformer for Image Captioning

Recent advancements of image captioning have featured Visual-Semantic Fusion or Geometry-Aid attention refinement. However, those fusion-based models, they are still criticized for the lack of geometry information for inter and intra attention refinement. On the other side, models based on Geometry-Aid attention still suffer from the modality gap between visual and semantic information. In this paper, we introduce a novel Geometry-Entangled Visual Semantic Transformer (GEVST) network to realize the complementary advantages of Visual-Semantic Fusion and Geometry-Aid attention refinement. Concretely, a Dense-Cap model proposes some dense captions with corresponding geometry information at first. Then, to empower GEVST with the ability to bridge the modality gap among visual and semantic information, we build four parallel transformer encoders VV(Pure Visual), VS(Semantic fused to Visual), SV(Visual fused to Semantic), SS(Pure Semantic) for final caption generation. Both visual and semantic geometry features are used in the Fusion module and also the Self-Attention module for better attention measurement. To validate our model, we conduct extensive experiments on the MS-COCO dataset, the experimental results show that our GEVST model can obtain promising performance gains.

==> 3_1_Data_Preparation_bkup.tex <==
As mentioned in Section~\ref{sec:Introduction},
our model is based on both the visual representation and semantic representation.

\noindent\textbf{Feature Preparation}. 
In order to model the given image in visual-level, each element $\vec{v_i}$ of visual feature vector $\matrix{V}$ is defined as the mean-pooled convolutional feature of the $i$-th salient region, which is a $d_v$-dimensional fixed-size feature vector (empirically set as $2048$). These visual features are extracted by means of the output of final convolution layer of \emph{Faster-RCNN} model~\cite{A_8}, which is widely used in previous work~\cite{B_4, B_5, B_6, B_7, B_8}.
Thus, for the visual information, we have $\matrix{V}=\{\vec{v}_{i}\}^{N_v}_{i=1}~(\vec{v}_{i}\in \mathbb{R}^{d_v})$ to denote the $N_v$-dimensional \emph{visual} feature vectors.
%
To fetch semantic representation for the given image, we consider to employ dense-caption model to obtain a list of dense-captions that are most likely to appear in the image.
Same to the work~\cite{D_1}, for each image, we get a list of dense-captions, corresponding confidence scores and bounding boxes information.
Then, each dense-caption will be encoded by a basic transformer encoder. Then, the confidence score will be used to assign a weight to each phrase. 
At last, we get a set of $d_s$-dimensional fixed-size semantic feature vectors, the $i$-th vector is denoted as ($\vec{s_i}$).
For the semantic information, we now have $\matrix{S}=\{\vec{s}_i\}^{N_s}_{i=1}~(\vec{s}_{i}\in \mathbb{R}^{d_s})$ to denote the $N_s$-dimensional \emph{semantic} dense-caption vectors.

\noindent\textbf{Geometry Entangled Matrix}. 
The inherent geometric structure among the input visual objects and semantic objects is beneficial for reasoning.
which, however, the geometric relation is hard to be extracted by the simple bounding box coordinates.
Therefore, we propose Geometry Entangled matrices, which take into account both inter- and intra- geometry relationships.
%
\begin{figure}
	%\centering
    \includegraphics[width=1\columnwidth, angle=0]{IEEE_TIP/IEEEtran/Image/3_1_Data_preparation_1.pdf}
	\vspace{-1ex}
	\caption{Detail of Geometry-Entangled feature generation. 
	The left one is an example of inter(visual-semantic) geometry relationships pair, 
	the blue rectangle stands for the bounding box for a corresponding dense-caption,
	the yellow rectangle stands for the bounding box for a corresponding salient object,
	$W_{(v,s)},H_{(v,s)}$ stand for the width and height of corresponding box. 
	The right one is an example of intra(visual-visual) geometry relationships pair, 
	there are three visual bounding boxes(blue, yellow, red) in the image. 
	$W_{(1,2,3)},H_{(1,2,3)}$ stand for the width and height of corresponding box.}
	\label{fig:Geometry_Entangle}
\end{figure}
%
%
As shown in the Figure \ref{fig:Geometry_Entangle}, for inter-geometry entangled matrix $\matrix{G_{v,s}^{inter}} \in \mathbb{R}^{N_v\times{N_s}\times{4}})$, 
given a semantic bounding box $B_s=(x_s, y_s, h_s, w_s)$ and a visual bounding box vector $B_v=(x_v, y_v, h_v, w_v)$, 
$x, y$ stand for the coordinate of the central point, 
$h, w$ stand for the height and width of the corresponding feature.
The inter-geometry entangled feature is $T_{v,s}=(T^{1}_{v,s}, T^{2}_{v,s}, T^{3}_{v,s}, T^{4}_{v,s})$, where each element is defined by that:
\begin{equation}
\begin{aligned}
& {T}^{1}_{v,s} = \log(\frac{|x_s-x_v|}{w_v}) \\
& {T}^{2}_{v,s} = \log(\frac{|y_s-y_v|}{h_v}) \\
& {T}^{3}_{v,s} = \log(\frac{w_s}{w_v})\\
& {T}^{4}_{v,s} = \log(\frac{h_s}{h_v})
\end{aligned}
\end{equation}
%
Each term stands for relative horizontal distance, relative vertical distance, width ratio and height ratio.

For intra-geometry entangled matrix $\matrix{G_{v,v}^{intra}} \in \mathbb{R}^{N_v\times{N_v}\times{5}})$, given three visual bounding box vectors
$B_{v,i}=(x_{v,i}, y_{v,i}, h_{v,i}, w_{v,i})$ where $i \in (1,3)$.
The intra-geometry entangled feature is $T_{v,v}=(T^{1}_{v,v}, T^{2}_{v,v}, T^{3}_{v,v}, T^{4}_{v,v}, T^{5}_{v,v})$, where each item is defined by that: 
\begin{equation}
\begin{aligned}
& {T}^{1}_{v,v} = \log(\frac{|x_i-x_j|}{w_i}) \\
& {T}^{2}_{v,v} = \log(\frac{|y_i-y_j|}{h_i}) \\
& {T}^{3}_{v,v} = \log(\frac{w_i}{w_j}) \\   
& {T}^{4}_{v,v} = \log(\frac{h_i}{h_j}) \\
& {T}^{5}_{v,v} = \log(\frac{N_c}{N_v})
\end{aligned}
\end{equation}
%
Where $N_v$ is the number of total visual features and $N_c$ is the number of visual features covered by the union bounding box of $B_{v,i}$ and $B_{v,j}$. The intuition is that, if the union box of $B_{v,i}$ and $B_{v,j}$. contains more other boxes, then it is less likely that $B_{v,i}$ and $B_{v,j}$ have a strong connection. As shown in the Figure \ref{fig:Geometry_Entangle}, $B_{v,1}, B_{v,2}, B_{v,3}$ stand for car, woman and motor, the union box of woman and car will cover the box of motor, but the union box of woman and motor will not fully cover the box of car, thus we think the woman is more likely to ride the motor rather than the car.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************

